Investigating the Nature of 3D Generalization in Deep Neural Networks

Visual object recognition systems need to generalize from a set of 2D training views to novel views. The question of how the human visual system can generalize to novel views has been studied and modeled in psychology, computer vision, and neuroscience. Modern deep learning architectures for object recognition generalize well to novel views, but the mechanisms are not well understood. In this paper, we characterize the ability of common deep learning architectures to generalize to novel views. We formulate this as a supervised classification task where labels correspond to unique 3D objects and examples correspond to 2D views of the objects at different 3D orientations. We consider three common models of generalization to novel views: (i) full 3D generalization, (ii) pure 2D matching, and (iii) matching based on a linear combination of views. We find that deep models generalize well to novel views, but they do so in a way that differs from all these existing models. Extrapolation to views beyond the range covered by views in the training set is limited, and extrapolation to novel rotation axes is even more limited, implying that the networks do not infer full 3D structure, nor use linear interpolation. Yet, generalization is far superior to pure 2D matching. These findings help with designing datasets with 2D views required to achieve 3D generalization. Code to reproduce our experiments is publicly available: https://github.com/shoaibahmed/investigating_3d_generalization.git

==> abstracts.tex <==

The question of how visual recognition systems should generalize to new views from a given set of views has been at the core of object recognition research for both humans as well as machine learning algorithms for decades.
This problem was traditionally solved via having an explicit 3D model of the object.
This distinction between developing a 3D model and matching is obscure for deep learning models, making it difficult to identify the behavior class these models adhere to.
These questions are of fundamental importance for both human vision and machine vision systems, but have been largely neglected by the deep learning community.
Motivated by prior work on human visual system, we attempt to understand the class of behavior deep learning models follow for recognition via studying the generalization capabilities of models on axis-aligned rotations of simple wire-like objects i.e. Paperclips as well as full 3D chairs.
Our results show that with a sufficient number of views, the model generalizes within the axis of rotation, but fails to generalize to rotations along a different axis.
This indicates that deep learning models leverages a mix of 2D and 3D matching i.e., it achieves generalization which is higher than pure 2D matching, but lower than that of having a full 3D model for recognition.
These results provide insight into the inner workings of deep networks and how it relates to classical work in computer vision and psychology.



Deep models are particularly effective at recognizing objects in real-world images.
However, the mechanisms at play are poorly understood.
A natural question that arises is: \textbf{how far can you generalize from a given set of training views for a 3D object?}
Classical work on computer vision has presented three different approaches to recognition: (i) full 3D matching where an object is matched with the full 3D model, (ii) pure 2D matching where the closest view from the training views is used for recognition, and (iii) recognition based on linear combination of views where the model interpolates between training views during matching.
In this paper, we attempt to analyze the generalization capabilities of the model from a given set of training views.
Furthermore, we evaluate which of these mechanisms is most plausible for recognition in deep networks.
For this purpose, we generate synthetic 3D wire-like objects i.e. Paperclips.
Our results show that with a sufficient number of views, the model generalizes within the axis of rotation, but fails to generalize to rotations along a different axis.
This indicates that the model performs recognition via a mix of 2D and 3D matching i.e., it achieves generalization which is higher than pure 2D matching, but lower than that of having a full 3D model for recognition.
These results provide insight into the inner workings of deep networks and how it relates to classical work in computer vision and psychology.




Visual object recognition systems need to generalize from a set of training views of an object to novel views of that object.
Improving the ability of a system to reliably generalize to novel views reduces the number of training examples required.
The question of how visual systems can generalize to novel views has been studied and modeled in psychology and classical computer vision.
Modern deep learning architectures for object recognition are clearly capable of generalizing to novel views, but the mechanisms and performance of that capability are not designed into the architecture explicitly and are not well understood.
In this paper, we measure the ability of common deep learning architectures to generalize across 3D views on object recognition tasks and compare the results with those of classic computer vision theories and results from human psychophysics.
We demonstrate that deep learning models show a strong ability to generalize to views around rotation axes represented in the training set.
Extrapolation to views beyond the range covered by views in the training set is limited, and extrapolation to novel rotation axes is even more limited, implying that the networks do not infer full 3D structure from training views despite having all necessary information for full 3D reconstruction available.
These results are of practical importance in two ways.
First, they allow us to design training sets for 3D object recognition with deep networks more efficiently.
Second, they imply that incorporating better 3D generalization capabilities into our deep networks may significantly improve the efficiency at which our networks use training data.

